Neuro-Inspired Information-Theoretic Hierarchical Perception for Multimodal Learning

Integrating and processing information from various sources or modalities are critical for obtaining a comprehensive and accurate perception of the real world in autonomous systems and cyber-physical systems. Drawing inspiration from neuroscience, we develop the Information-Theoretic Hierarchical Perception (ITHP) model, which utilizes the concept of information bottleneck. Different from most traditional fusion models that incorporate all modalities identically in neural networks, our model designates a prime modality and regards the remaining modalities as detectors in the information pathway, serving to distill the flow of information. Our proposed perception model focuses on constructing an effective and compact information flow by achieving a balance between the minimization of mutual information between the latent state and the input modal state, and the maximization of mutual information between the latent states and the remaining modal states. This approach leads to compact latent state representations that retain relevant information while minimizing redundancy, thereby substantially enhancing the performance of multimodal representation learning. Experimental evaluations on the MUStARD, CMU-MOSI, and CMU-MOSEI datasets demonstrate that our model consistently distills crucial information in multimodal learning scenarios, outperforming state-of-the-art benchmarks. Remarkably, on the CMU-MOSI dataset, ITHP surpasses human-level performance in the multimodal sentiment binary classification task across all evaluation metrics (i.e., Binary Accuracy, F1 Score, Mean Absolute Error, and Pearson Correlation).

==> Tables/tab_NoiseAdditionText.tex <==
\begin{table}[thbp]

% \vspace{0 cm}
\setlength{\abovecaptionskip}{0.2 cm}
\setlength{\belowcaptionskip}{-0. cm} 
\renewcommand{\arraystretch}{1.36}
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\setlength\tabcolsep{4pt}
    \begin{tabular}{M{1.36 cm}cM{0.86cm}M{1.26cm}M{1.26cm}M{1.26cm}M{1.26cm}M{1.26cm}M{1.26cm}}
    \hline
    \hline
    \textbf{Model} &
    \diagbox[width=1.86 cm]{\hspace{-5 pt}\raisebox{0.1ex}{$\boldsymbol{\textbf{Metrics}}$}}{\hspace{-16 pt}\lower0.2ex\hbox{$\boldsymbol{\sigma}$}} &
    - & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 \\ 
    \hline
    \multirow{2}[4]{*}{\textbf{MSDM}} & \textbf{Precision} & 0.719 & 0.711 (-1.11\%) & 0.709 (-1.39\%) & 0.707 (-1.67\%) & 0.704 (-2.09\%) & 0.700 (-2.64\%) & 0.688 (-4.31\%) \\
     & \textbf{Recall} & 0.714 & 0.705 (-1.26\%) & 0.702 (-1.68\%) & 0.700 (-1.96\%) & 0.695 (-2.66\%) & 0.691 (-3.22\%) & 0.679 (-4.90\%) \\
     \hline
    \multirow{2}[4]{*}{\textbf{ITHP}} & \textbf{Precision} & 0.753 & 0.751 (-0.27\%) & 0.748 (-0.66\%) & 0.747 (-0.80\%) & 0.746 (-0.93\%) & 0.743 (-1.33\%) & 0.740 (-1.73\%) \\
     & \textbf{Recall} & 0.752 & 0.750 (-0.27\%) & 0.745 (-0.93\%) & 0.743 (-1.20\%) & 0.742 (-1.33\%) & 0.740 (-1.60\%) & 0.736 (-2.13\%) \\
    \hline
    \hline
    \end{tabular}
\caption{\textbf{Evaluating Gaussian Noise Impact on Sarcasm Detection in Text Modality.} The table presents the weighted precision and recall for sarcasm detection on the MUStARD dataset, with an analysis of Gaussian noise addition to the text modality. Results are averaged over five cross-validation folds and 50 trials for each level of noise intensity. Each column indicates the standard deviation (represented by $\sigma$) of the introduced Gaussian noise with a mean of 0. Changes in performance metrics relative to the noise-free baseline are expressed as percentages.}
\label{tab:noise_addition_text}
\end{table}


==> Tables/tab_NoiseAdditionVideo.tex <==
\begin{table}[thbp]
% \vspace{0.2 cm}
\setlength{\abovecaptionskip}{0.2 cm}
\setlength{\belowcaptionskip}{-0.26 cm} 
\renewcommand{\arraystretch}{1.36}
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\setlength\tabcolsep{4pt}
    \begin{tabular}{M{1.36 cm}cM{0.86cm}M{1.26cm}M{1.26cm}M{1.26cm}M{1.26cm}M{1.26cm}M{1.26cm}}
    \hline
    \hline
    \textbf{Model} &
    \diagbox[width=1.86 cm]{\hspace{-5 pt}\raisebox{0.1ex}{$\boldsymbol{\textbf{Metrics}}$}}{\hspace{-16 pt}\lower0.2ex\hbox{$\boldsymbol{\sigma}$}} &
    - & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 \\ 
    \hline
    \multirow{2}[4]{*}{\textbf{MSDM}} & \textbf{Precision} & 0.719 & 0.709 (-1.39\%) & 0.705 (-1.95\%) & 0.702 (-2.36\%) & 0.698 (-2.92\%) & 0.692 (-3.76\%) & 0.683 (-5.01\%) \\
     & \textbf{Recall} & 0.714 & 0.703 (-1.54\%) & 0.700 (-1.96\%) & 0.694 (-2.80\%) & 0.689 (-3.50\%) & 0.678 (-5.04\%) & 0.668 (-6.44\%) \\
     \hline
    \multirow{2}[4]{*}{\textbf{ITHP}} & \textbf{Precision} & 0.753 & 0.748 (-0.66\%) & 0.745 (-1.06\%) & 0.743 (-1.33\%) & 0.742 (-1.46\%) & 0.739 (-1.86\%) & 0.735 (-2.39\%) \\
     & \textbf{Recall} & 0.752 & 0.745 (-0.93\%) & 0.741 (-1.46\%) & 0.740 (-1.60\%) & 0.738 (-1.86\%) & 0.733 (-2.53\%) & 0.730 (-2.93\%) \\
    \hline
    \hline
    \end{tabular}
\caption{\textbf{Evaluating Gaussian Noise Impact on Sarcasm Detection in Video Modality.} The table presents the weighted precision and recall for sarcasm detection on the MUStARD dataset, with an analysis of Gaussian noise addition to the video modality. Results are averaged over five cross-validation folds and 50 trials for each level of noise intensity. Each column indicates the standard deviation (represented by $\sigma$) of the introduced Gaussian noise with a mean of 0. Changes in performance metrics relative to the noise-free baseline are expressed as percentages.}
\label{tab:noise_addition_video}
\end{table}

